A Human-Centered Data-Driven Planner-Actor-Critic Architecture via Logic Programming

Recent successes of Reinforcement Learning (RL) allow an agent to learn policies that surpass human experts but suffers from being time-hungry and data-hungry. By contrast, human learning is significantly faster because prior and general knowledge and multiple information resources are utilized. In this paper, we propose a Planner-Actor-Critic architecture for huMAN-centered planning and learning (PACMAN), where an agent uses its prior, high-level, deterministic symbolic knowledge to plan for goal-directed actions, and also integrates the Actor-Critic algorithm of RL to fine-tune its behavior towards both environmental rewards and human feedback. This work is the first unified framework where knowledge-based planning, RL, and human teaching jointly contribute to the policy learning of an agent. Our experiments demonstrate that PACMAN leads to a significant jump-start at the early stage of learning, converges rapidly and with small variance, and is robust to inconsistent, infrequent, and misleading feedback.

==> eptcsdata.tex <==
\providecommand{\firstpage}{182}
\providecommand{\publicationstatus}{B. Bogaerts, E. Erdem, P. Fodor, A. Formisano,\\ 
G. Ianni, D. Inclezan, G. Vidal, A. Villanueva, \\
M. De Vos, F. Yang (Eds.): International \\
Conference on Logic Programming 2019 (ICLP'19).\\
EPTCS 306, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.306.23}{10.4204/EPTCS.306.23}}
\pdfoutput=1

